Modular Adaptation for Cross-Domain Few-Shot Learning

Adapting pre-trained representations has become the go-to recipe for learning new downstream tasks with limited examples. While literature has demonstrated great successes via representation learning, in this work, we show that substantial performance improvement of downstream tasks can also be achieved by appropriate designs of the adaptation process. Specifically, we propose a modular adaptation method that selectively performs multiple state-of-the-art (SOTA) adaptation methods in sequence. As different downstream tasks may require different types of adaptation, our modular adaptation enables the dynamic configuration of the most suitable modules based on the downstream task. Moreover, as an extension to existing cross-domain 5-way k-shot benchmarks (e.g., miniImageNet -> CUB), we create a new high-way (~100) k-shot benchmark with data from 10 different datasets. This benchmark provides a diverse set of domains and allows the use of stronger representations learned from ImageNet. Experimental results show that by customizing adaptation process towards downstream tasks, our modular adaptation pipeline (MAP) improves 3.1% in 5-shot classification accuracy over baselines of finetuning and Prototypical Networks.

==> Modular Adaptation ICCV2021 - Arxiv/ch/00-Abstract.tex <==
\begin{abstract}

Adapting pre-trained representations has become the go-to recipe for learning new downstream tasks with limited examples. While literature has demonstrated great successes via representation learning, in this work, we show that substantial performance improvement of downstream tasks can also be achieved by appropriate designs of the adaptation process. Specifically, we propose a modular adaptation method that selectively performs multiple state-of-the-art (SOTA) adaptation methods in sequence. 
As different downstream tasks may require different types of adaptation, our modular adaptation  enables the dynamic configuration of the most suitable modules based on the downstream task. % through hyperparameter search. 
%By studying which set of modules are effective for which downstream tasks, we show that domain difference between pretext and downstream tasks is more than just being similar or not. Difference in label ontology and image style may require special treatment during adaptation. As such, 
Moreover, as an extension to existing cross-domain 5-way k-shot benchmarks (e.g., miniImageNet $\rightarrow$ CUB), we create a new high-way (\~{}100) k-shot benchmark with data from 10 different datasets. This benchmark provides a diverse set of domains and allows the use of stronger representations learned from ImageNet. Experimental results show that by customizing adaptation process towards downstream tasks, our modular adaptation pipeline (MAP) improves 3.1\% in 5-shot classification accuracy over baselines of finetuning and Prototypical Networks.

\end{abstract}

==> Modular Adaptation ICCV2021 - Arxiv/ch/01-Intro.tex <==
%\vspace{-2mm}
\section{Introduction}
%\vspace{-1mm}

\begin{figure*}[t]
    \centering

    \includegraphics[width=1.0\textwidth]{fig/01-teaser.pdf}
    %\vspace{-2mm}
    \caption{Block diagram of our proposed modular adaptation pipeline (MAP). MAP dynamically selects the most appropriate modules and their hyperparameters based on the characteristics of the given downstream task. MAP applies these selected modules in sequence to adapt the pre-trained models towards the target downstream task.}    
    \label{fig:teaser}
    %\vspace{-2mm}
\end{figure*}


In few-shot learning (FSL), the task of building models using limited examples, adapting pre-trained representations has demonstrated successful applications in computer vision and natural language processing~\cite{fei2006one,vinyals2016matching,ravi2016optimization,hariharan2017low}. Finetuning pre-trained networks and learning classifiers on top of these embeddings leads to highly accurate classifiers even for data scarce conditions. An ideal pre-trained representation to start with is one that is learned in domains relevant to the target task or sufficiently diverse to enable effective transfer. However, in practice, relevant data is scarce and there is often a certain degree of domain shifts between the pretext and downstream tasks, where label ontology, viewpoint, image style, and/or input modality may differ. 
As such, cross-domain FSL~\cite{triantafillou2019meta,guo2020broader,tseng2020cross} recently brings renewed interest to this classical transfer learning problem focusing on the low data regime.

%When trying to overcome the domain gap in cross-domain few-shot learning, 
Existing studies show that depending on the characteristics of the underlying domain shifts, different downstream tasks may favor different adaptation methods, either finetuning-based~\cite{chen2019closer,guo2020broader} or metric learning-based approaches~\cite{tian2020rethinking,chen2020new}. 
For finetuning-based methods, the degree of finetuning required may also depend on the domain differences~\cite{li2020rethinking,cai2020cross,guo2019spottune} and the amount of training data available in the target domain~\cite{kolesnikov2019big}.
%Specialized methods have been developed to exploit object localization and part-whole relationships, but may not be straightforward to apply to domains without such patterns. 
As a result, developing a one-size-fits-all cross-domain FSL approach has been challenging, if not entirely infeasible. To facilitate the appropriate design of cross-domain few-shot algorithms, a deeper understanding of domains, algorithms and their relationships is critical. 

In this work, we propose a modular approach for cross-domain few-shot adaptation that can be dynamically customized based on domain characteristics as an alternative to commonly used one-size-fits-all solutions. We refer to our method as the Modular Adaptation Pipeline (MAP, Figure~\ref{fig:teaser}). To build MAP, we first standardize few-shot adaptation methods into modules, where each module takes as the input a model and the adaptation datasets, and produces an adapted model as the output. 
We chain these modules into a consolidated pipeline, where multiple adaptation methods are applied in sequence. Given a downstream task, which adaptation modules should be applied as well as the hyperparameters of each selected module can be flexibly configured and automatically optimized via Bayesian optimization.

MAP can, thus, be considered as applying different loss terms according to the chosen methods sequentially to progressively adjust the input model towards the target downstream task. 
MAP enables flexible and customized integration of various SOTA techniques, whereas schemes based on joint optimization with an integrated loss function (e.g., weighted combination of multiple loss terms) may find it difficult to accommodate such diverse methods. Furthermore, while, in theory, our modular approach sacrifices global optimality due to step-wise optimization, schemes based on joint optimization, in practice, may also find it difficult to arrive at the global optima
simply because of the complexity of the loss landscape, which can be further complicated by the involvement of module hyper-parameters. As a result, our modular and sequential approach stands in contrast to methods based on joint optimization as an arguably better design choice for practical problems.  

As an exemplar realization of MAP, we integrate a collection of metric-based, finetuning, semi-supervised, and domain adaptation methods such as Prototypical Networks~\cite{snell2017prototypical,chen2020new}, batchnorm tuning~\cite{guo2020broader}, FixMatch~\cite{sohn2020fixmatch}, power transform, and semi-supervised embedding propagation~\cite{hu2020leveraging,ye2020hybrid}. This allows us to study their importance in different cross-domain few-shot adaptation tasks, providing empirical insights for a deeper understanding of adaptation algorithms, domain characteristics, and their relationships. 
%We are able to identify two promising adaptation pipelines, referred to as the H-domain-real-5 and H-domain-real-10, that specialize in low-shot and medium-shot cross-domain learning respectively, each comprised of different adaptation methods. 

Our major contributions include: 

1) We introduce a modularized approach for cross-domain few-shot adaptation to integrate a wide range of SOTA adaptation methods and apply them in sequence. In comparison to one-size-fits-all solutions, our method can dynamically select a sequence of the most suitable modules based on the characteristics of downstream tasks. In comparison to solutions based on joint optimization with combined losses, our method can work with a more diverse set of adaptation methods and achieve a balanced capability between finding the (sub)optimal solution and handling complex loss landscape. 

2) Our empirical analysis on the cross-domain performance of MAPs optimized for different domains shed insightful light on the similarities among downstream tasks, which varies depending on domain shifts and the availability of training data. 
%modules used in dataset-specific adaptation pipelines reveals multiple dimensions of the domain characteristics in real datasets. 

3) We show that by customizing the adaptation process based on the target domain and availability of training examples, MAP produces on average a 3.1\% improvement in 5-shot classification accuracy over few-shot and finetuning baselines on a large-scale 100-way ImageNet $\rightarrow$ 10 datasets benchmark. 



==> Modular Adaptation ICCV2021 - Arxiv/ch/02-Related.tex <==
%\vspace{-1mm}
\section{Related work}
%\vspace{-1.5mm}
\subsection{Cross-domain few-shot learning}
%\vspace{-1.5mm}
 SOTA FSL approaches use a combination of representation learning for improving the pre-trained representation~\cite{tian2020rethinking,chen2020new,mangla2020charting,gidaris2019boosting,ye2020hybrid,chen2019self}, meta-learning for building more generalizable pre-trained models via episodic training~\cite{vinyals2016matching,finn2017model,snell2017prototypical}, and flexible adaptation such as prototype-based~\cite{ren2018meta,hu2020leveraging} and graph-based~\cite{satorras2018few,liu2018learning}. 
FSL benchmarks to date often split datasets into two disjoint sets of classes, one for pre-training and the other for adaptation. In practice, however, we often need to adapt SOTA pre-trained representations to learn classifiers using limited training examples on a different domain. Studies show that approaches designed for same-domain few-shot learning may not perform better than simple finetuning when there is a large domain gap between the pretext and downstream tasks~\cite{chen2019closer,guo2020broader}.
As such, recent works~\cite{triantafillou2019meta,guo2020broader,tseng2020cross} start to design more effective cross-domain FSL algorithms and more realistic cross-domain FSL benchmarks. 

Our modular adaptation approach focuses on cross-domain few-shot adaptation and advances existing work by providing a framework for integrating various adaptation methods. 
We show that cross-domain FSL approaches could benefit from customizing the adaptation algorithm towards the target domain through hyperparameter adaptation. 
We also introduce a larger-scale cross-domain FSL benchmark that adapts ImageNet pre-trained representations for downstream tasks with more classes (100-way vs. existing 5-way) to bridge the gap between existing small-scale cross-domain FSL benchmarks and the needed large-scale transfer learning.

%Relavant papers
%SELF-TRAINING FOR FEW-SHOT TRANSFER ACROSS EXTREME TASK DIFFERENCES
%BOIL: TOWARDS REPRESENTATION CHANGE FOR FEW-SHOT LEARNING
%Explain and Improve: Cross-Domain Few-Shot-Learning Using Explanations

\subsection{Adaptation methods in transfer learning}
%Works on Finetuning: Spottune, Smart L2 regularization

In transfer learning, a variety of approaches for adaptating pre-trained classifiers to downstream tasks have been developed, such as fine-grained control of finetuning~\cite{li2018explicit,guo2019spottune} and network scaling~\cite{wang2017growing,kolesnikov2019big}. 
%While many approaches are designed for large-scale adaptation problems, many may conditionally apply to cross-domain FSL. 
However, studies have shown that their performance depends heavily on hyperparameters, which may vary substantially according to the dataset size and the domain gap~\cite{li2020rethinking}. 

In contrast, our work shows that multiple adaptation methods and their hyperparameters can be configured under few-shot settings through cross validation and by transferring hyperparameters from similar tasks. This paves a distinctive path for integrating sophisticated adaptation methods in a more robust manner.

\subsection{Automatic transfer learning}

Inspired by the successes of automatic machine learning (AutoML), automatic transfer learning (i.e., automatically building models for new downstream tasks while leveraging models trained on pretext tasks) has gained increasing interests.
Relevant work includes automatically identifying relevant sources ~\cite{zamir2018taskonomy,Yan_2020_CVPR}, pre-trained model selection and empirical selection of hyperparameters for transfer learning~\cite{kolesnikov2019big,li2020rethinking}.

Our work focuses on the automated selection of adaptation methods along with their hyperparameters. The cross-domain performance of domain-specific MAPs can also be used as a post-hoc criterion for source selection. 

%suggests that there is room of improvements in developing more sophisticated adaptation process and automatically configure it towards the target dataset. Effectiveness of adaptation procedures on different datasets may also provide a different perspective of task relevance.



==> Modular Adaptation ICCV2021 - Arxiv/ch/03-Approach.tex <==
\section{Approach}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.00\textwidth]{fig/02-pipelines.pdf}
    \caption{An exemplar realization of MAP based on seven adaptation methods of different types including FSL, domain adaptation (DA), finetuning and semi-supervised learning. These modules are chained sequentially with a fixed ordering and can be ``switched off'' using a skip connection. ProtoNet for FSL and finetuning for transfer learning can be implemented as special cases of MAP.}
    \label{fig:pipeline}
\end{figure*}


%-- Setup --

In this work, we focus on the problem of adapting a pre-trained model to perform image classification on a different dataset in a new domain (i.e., the target domain). Specifically, given 1) a pre-trained image classifier $F$ 
%consisting of an embedding network $E$ and a classifier $C$ 
which takes in an image $I$ and outputs scores of classes $s=F(I)$, 2) an N-way K-shot labeled training set $D_l$, and 3) a set of unlabeled samples in the target domain $D_u$, the task is to build an updated image classifier $F'$ in the target domain to predict categories of testing samples. 

At the meta level, an adaptation approach can be abstracted into a module $F'=M(F,D_l,D_{u})$ or equivalently in operator form $F'=M(D_l,D_{u}) \circ F$. Multiple modules can be chained for a composite adaptation approach.
\begin{align*}
F' &= \underbrace{M_n (D_l,D_{u})\circ \cdots \circ M_1 (D_l,D_{u})}_{\text{n modules}} \circ F \\
&\triangleq M(D_l,D_u) \circ F
\end{align*}
Chaining multiple modules corresponds to adapting a pre-trained model using a collection of adaptation methods sequentially. In this work, we propose one such design, namely MAP, and study the benefits and challenges in constructing ``pipelined'' adaptation methods. 

We treat the configuration that switches on and off adaptation methods as additional hyperparameters to be learned during training. These configuration parameters are learned jointly with the hyperparameters of each selected module. While transfer learning and meta-learning have studied adapting model parameters to downstream tasks, adapting hyperparameters remains an under-explored area. 
However, hyperparameters should be adapted to the target domain, since studies indicate that the optimal effective learning rate in finetuning~\cite{kolesnikov2019big,li2020rethinking} and the effectiveness of different types of adaptation algorithms~\cite{triantafillou2019meta,chen2019closer,guo2020broader} both depend on domain similarity and the amount of training data. In this regard, MAP not only searches for the most suitable modules but also their hyperparameters for improved domain transfer. 

%Given a downstream task, hyperparameters in an MAP such as which modules should be applied, and the hyperparameters of the active modules may be learned through cross-validation. 
%MAP leads to a large hyperparameter search space for adaptation. 
Combining multiple adaptation methods via learnable configuration leads to a large search space, where traditional gradient descend may find difficult to handle. %The space of reachable image classifiers through MAPs may go beyond gradient descend on a given architecture. 
To fully leverage the potential of MAP, we design a simple yet effective protocol to learn hyperparameters based on cross validation and transferring hyperparameters across tasks. 

%How often can optimal MAP be learned and how often does hyperparameter learning overfit and decrease performance are interesting questions to explore.

In Section 3.1 and 3.2, we introduce the design space of our MAP including its building blocks and pipeline. We describe the proposed MAP search protocol in Section 3.3.

\subsection{Building blocks}

We implement seven modules based on adaptation methods with demonstrated successes in literature. The goal is to cover a diverse set of techniques such as FSL, domain adaptation and semi-supervised learning. A full list of options provided by each module is available in Appendix~\ref{sec:module_details}. 

\paracompact{Finetuning.} Finetune both the encoder (i.e., networks that map the input to an embedding feature space) and the classifier layers. The choice of optimizer (e.g., Adam or SGD), learning rate, momentum, weight decay, data augmentation, batch size, number of epochs and learning rate stepping schedule are set as hyperparameters. We also included the option of re-initializing the classification network with a fully connected layer. 

\paracompact{Transductive ProtoNet (TransPN).} Prototypical Networks with scaled cosine distance~\cite{chen2020new}, embedding power scaling~\cite{hu2020leveraging}, and CIPA~\cite{ye2020hybrid} prototype propagation for transductive learning. These algorithms have been shown to reach SOTA on FSL datasets. The cosine distance scaling factor, power scaling factor and the toggle of transductive learning are part of the hyperparameters. TransPN reduces the classification layer to simply comparing the embedding of a test sample against class prototypes based on scaled cosine similarity.

\paracompact{Finetuning batchnorm layer (TuneBN).} Updating batchnorm statistics with unlabeled data from the target domain helps model adaptaion in few-shot settings~\cite{nichol2018first,guo2020broader}. Network weights are frozen while batches of unlabeled data are passed through the network to update batchnorm statistics. TuneBN also serves the role of setting the momentum of batchnorm layers of the input network, which is an important factor in adaptation.

\paracompact{Semi-supervised learning with pseudo labels (SSL-PseudoLabel).} High-confidence predictions on unlabeled data are used as ``pseudo labels'' along with groundtruth labels during training~\cite{lee2013pseudo}. 

\paracompact{Semi-supervised learning with entropy minimization (SSL-Entropy).} Entropy on unlabeled examples is used as an additional loss term during training~\cite{grandvalet2005semi}.

\paracompact{Semi-supervised learning with student-teacher (SSL-MeanTeacher).} A semi-supervised learning approach that uses predictions from a running average network as the ``mean teacher'' to regularize the training of a student network~\cite{tarvainen2017mean}.

\paracompact{Semi-supervised learning with FixMatch (SSL-FixMatch).} Use consistency between strongly and weakly augmented inputs for semi-supervised learning~\cite{sohn2020fixmatch}. 

 


\subsection{Pipeline design}


Figure~\ref{fig:pipeline} depicts an exemplar realization of our MAP. It consists of 11 modules. Finetuning is followed by semi-supervised learning with BatchNorm and ProtoNet modules in-between. Each module can be switched on or off. When switched off, a module is replaced with a skip connection, i.e., $F'=F$. 
While our empirical pipeline design does not cover all possible combinations of the building blocks, it supports a rich and compact set of configurations for selecting various methods. It covers standard baselines such as BatchNorm + ProtoNet and BatchNorm + finetuning. It also follows best practices such as finetuning the network before semi-supervised learning. 

The search space of hyperparameters consists of switches, $\{\text{on},\text{off}\}^n$, and the hyperparameters for each module, 126 hyperparameters in total. By keeping the number of modules in our pipeline fixed, standard Bayesian hyperparameter search techniques can be used to optimize MAP given a downstream task. 
Neural architecture search~\cite{zoph2016neural} and hyperparameter search transfer learning~\cite{perrone2018scalable} may enable further expansion of the search space and potentially result in better pipelines. In this work, we focus on studying the feasibility and impacts of MAP and leave the aforementioned further improvements to future work.


\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{fig/03-datasets.pdf}
    \caption{Example images in our ImageNet $\rightarrow$ 10 datasets cross-domain FSL benchmark. The datasets cover a wide variety of qualitatively different domains to assist the development of few-shot adaptation approaches.}
    \label{fig:dataset}
\end{figure*}

\subsection{Search protocol}

Given a downstream task $\{D_l,D_{u}\}$, the goal of domain dependent adaptation is to obtain an optimal set of MAP hyperparameters. The standard approach is to optimize $k$-fold cross validation performance: first construct multiple cross validation splits by randomly dividing $D_l$ into training splits $D^{train,i}_l$ and validation splits $D^{val,i}_l,i=1,\ldots,k$, and then perform adaptation on $\{D^{train,i}_l,D_u\}$ and optimize performance on $D^{val,i}_l$ using Bayesian hyperparameter optimization. Herein, the large search space presents a major challenge. For our exemplar MAP with 11 modules, there are $2^{11}=2,048$ possibilities in just deciding which modules should be turned on. From our experiments, we find that MAP optimization from scratch typically requires $>$300 iterations to converge, which often takes days on a single GPU. As reference, finetuning and ProtoNet, on the other hand, often converge within 30 iterations. 

To speed up MAP optimization, we propose to transfer MAP hyperparameters across domains. Intuitively, a MAP optimized for one adaptation problem may also perform well on similar problems with similar requirements. It, therefore, could serve as a better starting point of hyperparameter search than from scratch. A set of MAPs optimized for a diverse set of domains could readily cover a large variety of adaptation problems so that satisfactory performance could be reached by simply selecting the best performing MAP out of the set for a given new downstream task.

Specifically, we first collect an initial set of 20 to 50 high-performing MAPs on N-way K-shot adaptation tasks sampled from a diverse collection of datasets (excluding the target dataset), by running MAP hyperparameter search from scratch for 500 iterations. Building the initial collection of MAPs may take weeks across multiple GPUs. However, during adaptation, only MAPs in the collection are evaluated on the crossval splits $\{D^{train,i}_l,D_u\}$ and $D^{val,i}_l$ to select the most suitable MAP for the given downstream task. We show in experiments that transferring with a set of MAPs reaches similar accuracy as searching from scratch most of the times but converges more than 10$\times$ faster. 

Our search protocol is related to hyperparameter transfer learning~\cite{perrone2018scalable} and BiT-Hyperrule~\cite{kolesnikov2019big}, an empirical rule for determining finetuning hyperparameters. Different from~\cite{perrone2018scalable} which learns a transferable embedding space of hyperparameters, our approach simply finds hyperparameters that addresses a diverse set of tasks. MAP creates a more extended hyperparameter space than finetuning, which may open opportunities for deriving more sophisticated domain-dependent hyperparameter rules.



==> Modular Adaptation ICCV2021 - Arxiv/ch/04-Experiment.tex <==
%\vspace{-0.5mm}
\section{Experiment}
%\vspace{-0.5mm}
\subsection{Experimental Setup}
%\vspace{-0.5mm}
\input{fig/table01-main}

\paracompact{Dataset.}
SOTA FSL has benefited from improving pre-trained representations on miniImageNet~\cite{vinyals2016matching,ravi2016optimization,triantafillou2019meta} through improved architectures~\cite{hariharan2017low,qiao2018few}, episodic meta-training~\cite{finn2017model,chen2020new}, knowledge distillation~\cite{tian2020rethinking} and self-supervised learning~\cite{gidaris2019boosting,mangla2020charting,ye2020hybrid}. Improvements on miniImageNet representations have been shown to be orthogonal to improvements in few-shot adaptation~\cite{hu2020leveraging,ye2020hybrid}, but are to certain degree disconnected from the representation learning community where the focus is on ImageNet~\cite{kolesnikov2019big,touvron2020training,radosavovic2020designing,chen2020simple} and beyond~\cite{dosovitskiy2020image}. 
To fully benefit from representation learning, we introduce a new large-scale 100-way 2- to 20-shot ImageNet $\rightarrow$ 10 datasets benchmark for cross-domain few-shot learning. 
These 10 adaptation datasets include DomainNet-\{real, clipart, sketch, quickdraw, infograph, painting\}~\cite{peng2019moment}, CIFAR-100~\cite{krizhevsky2009learning}, DTD-textures~\cite{cimpoi14describing}, FGVC-aircraft~\cite{maji13fine-grained} and GTSRB-traffic signs~\cite{Stallkamp2012}. Figure~\ref{fig:dataset} illustrates example images from the respective datasets. 
The choice of datasets is inspired by the VTAB ~\cite{zhai2019visual} and MetaDataset~\cite{triantafillou2019meta} benchmarks but with focus on fixed-way fixed-shot to study domain-dependent adaptation strategies.


All classes in the respective datasets are used except for DomainNet, where only the top 100 most frequent classes are used as there are insufficient testing examples for categories towards the tail of the class distribution. We randomly sample images to create K$\in$\{2,5,10,20\}-shot adaptation tasks with 20 test examples per class. The process is repeated over 5 random seeds to create 5 splits for each of the N-way K-shot problem. Accuracy is reported per-dataset per-shot, averaged over the 5 random splits. Following existing FSL conventions, unlabeled test examples are available for semi-supervised and/or transductive learning~\cite{ren2018meta,liu2018learning}. 
The splits are available at \url{https://github.com/frkl/modular-adaptation}.

We also benchmark our approach using existing cross-domain few-shot datasets including the VL3 challenge~\cite{guo2020broader} (5-way 5- to 20-shot miniImageNet $\rightarrow$ CropDisease~\cite{mohanty2016using}, EuroSAT~\cite{helber2019eurosat}, ISIC~\cite{codella2019skin} and ChestX~\cite{wang2017chestx}) and the four datasets from the LFT work~\cite{tseng2020cross} (5-way 1-\&5- shot miniImageNet $\rightarrow$ CUB~\cite{WahCUB_200_2011}, Cars~\cite{KrauseStarkDengFei-Fei_3DRR2013}, Places~\cite{zhou2014learning} and Plantae~\cite{van2018inaturalist}).

\paracompact{Backbone architecture.} We focus on adaptation from publicly available standard backbones for each benchmarking datasets. For VL3 and LFT, we used the baseline ResNet-10 pre-trained on miniImageNet provided by~\cite{cai2020cross}
\footnote{https://github.com/johncai117/Meta-Fine-Tuning} 
and ~\cite{tseng2020cross}
\footnote{https://github.com/hytseng0509/CrossDomainFewShot}
, respectively. For our ImageNet $\rightarrow$ 10 datasets settings, we used an EfficientNet-B0~\cite{tan2019efficientnet} pre-trained on ImageNet provided by the EfficientNet-pytorch model zoo\footnote{https://github.com/lukemelas/EfficientNet-PyTorch}. Input image resolutions are $224 \times 224$. 
%By default without data augmentation, images are resize to input resolution without preserving the aspect ratio. 

\paracompact{Baselines.} We choose two baselines 1) finetuning (FT) where only TuneBN and finetuning modules are enabled and 2) prototypical networks (PN) where only TuneBN and Transductive ProtoNet modules are enabled as illustrated in Figure~\ref{fig:pipeline}. These two baselines are selected as their search space can sufficiently cover SOTA cross-domain few-shot adaptation techniques. 

\paracompact{Search strategy.} Hyperparameters are determined through 5-split cross validation on the adaptation set (each split with 50\% training and 50\% validation). As described in Section 3.3, to save computations of online adaptation%, we do not necessary need to perform pipeline optimization on the full search space. Instead
, we start from a set of pre-selected high-performing 1-, 2-, 5- and 10-shots pipelines on the 10 adaptation datasets\footnote{Using HyperOPT https://github.com/hyperopt/hyperopt}, total 40 pipelines for a reduced search space and, thus, decreased online computational complexity. Accordingly, we compare two hyperparameter selection strategies, one with the set of pre-selected pipelines (referred to as the \emph{transfer} setting), and the other with a set of best-performing pipelines optimized for lower shots on the adaptation dataset to approximate hyperparameter search from scratch (referred to as the \emph{from-scratch} setting). To verify the effectiveness of cross validation, we also design a third \emph{oracle} setting where hyperparameters are searched and evaluated directly on test data. For example, for 10-shot CIFAR-100 experiments, the \emph{transfer} setting selects pipelines from 1-, 2-, 5- and 10-shots from other datasets such as DomainNet-Clipart. The \emph{from-scratch} setting uses the pipelines optimized for 1-, 2-, and 5-shots on CIFAR-100. The \emph{oracle} setting uses the pipeline for 10-shot on CIFAR-100. 
 
%We study the effectiveness of our hyperparameter transfer protocol by comparing 1) from scratch: searching MAPs from scratch using hyperopt for 500 rounds; 2) transfer: selecting from the best MAPs searched on all the remaining datasets for [1,2,5,10]-shots. We also study oracle: finding the best MAP on the adaptation/test sets directly using 500 rounds of hyperparameter search as an upperbound. A detailed list of hyperparameter search spaces for FT, PN and Full can be found in [appendix].
%MAPs under the \emph{from scratch} setting is computational intensive and require about 48-720 GPU hours depending on dataset size of the downstream tasks. 
%To reduce compute time we reuse hyperparameters searched on the first split for the remaining splits. 
%Note that for 1-shot scenarios without enough examples for cross-validation, we manually set the hyperparameters and the same set of hyperparameters is used across all datasets.

%\vspace{-3mm}
\subsection{Experimental results}
%\vspace{-1mm}


\paracompact{Comparison against baselines.} Table 1 compares the performance of MAP vs. baselines (i.e., PN, FT) on the ImageNet $\rightarrow$ 10 datasets cross-domain task. Between PN and FT, we observe that PN, a FSL method, and FT, a transfer learning method, performs better on lower-shots (i.e., 2-shot) with similar domain and higher-shots (i.e., 5-, 10-, 20-shots) with disjoint domain, respectively, This agrees with the underlying designs of these methods and the general observations in literature. Thanks to its modularized design that supports online pipeline reconfiguration, MAP on average outperforms both PN and FT for 2-, 5-, 10-shots by 3.96\%, 3.13\% and 1.04\%, respectively. For 20-shot, MAP achieves comparable performance as FT. As the number of shots increases, the performance gain achieved by MAP degrades. This is expected since in general FT outperforms few-shot methods given sufficient labeled data.  
\input{fig/table04-vl3-lft}


In Table 1, DomainNet domains are arranged based on their realism with QDraw being the most abstract and Real the most realistic. Studying the performance across these domains, we notice that adaptation accuracy improves as the domain becomes more realistic. This is because the source domain is ImageNet. MAP achieves improved performance for all the domains except for QDraw, indicating that MAP's step-wise sequential optimization may be trapped into local optima at the earlier stage of the pipeline for scenarios with a large disparity between the source and target domains.  

%\paracompact{MAP significantly improves performance on $\le$10 shot.} Comparing PN and FT [from-scratch] on [our benchmark] echoes the finding of existing works, that PN performs better on few-shot, where as for $\ge$5-shot FT starts to outperform PN. PN also performs better on DomainNet-Real dataset relative to other datasets, which indicates that PN tends to be more effective for small domain shifts. 
%However, MAP significantly , averaged across all datasets. 

%Interestingly, on all datasets except for DomainNet-Quickdraw, MAP performs better than the best of PN and FT, confirming the existence of a class of effective hybird PN-FT adaptation approaches for cross-domain few-shot learning. It shows that while FT is a consistent performer in cross-domain few-shot learning, it could still be complemented by prototype-based methods. 

%In addition, the gains from MAP tend to be larger for large domain shifts. The benefit from adding PN to FT seems to go beyond small domain gap cases which PN excels at. 

%Performance gains from MAP diminishes on high-shot, which is expected as the transfer from ImageNet becomes less effective.

%\paracompact{Results on VL3 and LFT.}
We compare the performance of our MAP against existing approaches using the same backbone architectures on the LFT (Table~\ref{table:LFT}) and VL3 (Table~\ref{table:VL3}) cross-domain FSL benchmarks.\footnote{Additional implementation details are available in Appendix~\ref{sec:lft_vl3_details}.} We achieve competitive performance against SOTA on the small-scale 5-way datasets, especially for the LFT benchmark. Notably, on ISIC and ChestX in the VL3 benchmark, which are datasets of medical imagery, MAP performance is still relatively lower than the baselines. This is because our exemplar MAP does not include strong domain adaptation modules (the only domain adaptation comes from BatchNorm). By incorporating additional domain adaptation modules, we expect MAP performance to be further improved on these two datasets. 
%Despite that we are changing only the adaptation component and reusing MAPs for EfficientNet on ResNet-10, we achieved  and much higher performance against baseline methods on LFT. This shows that MAPs could be scaled to both small and large problems. 


\input{fig/table02-summary}


\paracompact{Comparison across search strategies.} Table 2 compares averaged performance of PN, FT, MAP across the six domains in DomainNet under the \emph{from-scratch}, \emph{transfer}, and \emph{oracle} settings for 2-, 5-, 10-, and 20-shots.\footnote{Accuracy on each domain is available in Appendix~\ref{sec:full_results}.} Our experiments under the \emph{oracle} setting show that the improvement margin between MAP and PN/FT on DomainNet is approximately $4.04\%$, $2.72\%$, and $0.85\%$, for 2-, 5-, and 10-shots, respectively. MAP under both \emph{from-scratch} and \emph{transfer} settings has achieved such improvement, suggesting that despite the large number of additional parameters introduced by dynamic pipeline configuration, MAP seems not yet suffer from over-fitting (i.e., similar improvement is achieved on the holdout fold of cross-validation). This allows for a larger search space by adding more modules into the MAP pipeline (e.g., self-supervised learning).   
%Comparing Full vs FT and PN across oracle hyperparameters, we see that MAP creates 4\%, 3\% and 1\% theoretical performance headroom for further performance improvements. The headroom has been fulfilled almost exactly by [from-scratch] and [transfer] hyperparameter search strategies. The vast number of additional hyperparameters introduced by MAP did not bring any meta-overfitting side effect. This suggests that the research on better adaptation methods could still focus on improving the headroom, such as introducing more modules to MAP -- perhaps domain-specific -- without worrying about meta-overfitting.



Comparing between \emph{from-scratch} and \emph{transfer}, \emph{transfer} achieves similar performance to \emph{from-scratch}. The fact that the performance difference is marginal also verifies our conjecture that initializing from a set of pre-selected pipelines is a practical and effective alternative to searching the whole parameter space for reduced online computation. 
Figure~\ref{fig:hp_convergence} shows the convergence rate of \emph{transfer} against vanilla Bayesian hyperparameter search on 5-shot DomainNet-Clipart, where \emph{transfer} yields an approximately $20\times$ reduction in online computation.

%our [transfer] strategy seems to match from-scratch hyperparameter search on Full and FT despite using 20x less budget during adaptation. 

%Performance is very close to oracle or sometimes even better - because oracle is generated through 500 rounds of hyperparameter search and may not be sufficient to find the best pipeline. 

\begin{figure}[t]
\centering
%\vspace{-10pt}
\includegraphics[width=0.75\textwidth]{fig/04-hp-transfer.pdf}
\caption{MAP convergence rate on a DomainNet-Clipart 5-shot task. \emph{transfer} converges within 20 evaluations, whereas vanilla Bayesian hyperparameter optimization requires more than 200 evaluations to converge.}%
\label{fig:hp_convergence}
\end{figure}


\paracompact{Comparison across domains.} The domain-specific nature of MAPs allows for the study of which domains favors which adaptation methods. 
%Despite a simple picture that oracle performance has been achieved, choosing the right hyperparameters plays an important role in achieving good performance with MAPs. 
Table~\ref{table:pipeline_generalization} shows the cross-domain performance of six MAPs optimized for 5-shot on Domain-QDraw, -Infgrph, -Sketch, -Clipart, -Pnting, and -Real. In general, the best performance is achieved using the MAP optimized for the same or similar domains. Figure~\ref{fig:pipelines_dn} visualizes the MAPs optimized for DomainNet-Clipart-5 and DomainNet-QDraw-5. Both pipelines start from a ProtoNet initialization and perform semi-supervised finetuning. However, DN-Clipart-5 seems to emphasize FSL with TransPN as the output classifier, whereas DN-QDraw-5 relies more on finetuning with larger learning rates. This again verifies our conjecture that different domain characteristics favor different adaptation techniques and the need of adaptive configuration of these methods. 

%The Map optimized for DomainNet-Clipart seems to generalize well to other painting-like domains, whereas the DN-QDraw-5 pipeline is specifically effective on the Domain-Quickdraw dataset. This shows that MAPs may indeed need to be domain-specific to reach optimal performance. 


\input{fig/table03-generalization}

\begin{figure}[t]
\centering
\includegraphics[width=1.0\textwidth]{fig/05-pipelines-dn.pdf}
\caption{MAPs optimized for 5-shot on DomainNet-Clipart (top) and DomainNet-QDraw (bottom).}%
\label{fig:pipelines_dn}
\end{figure}


The cross-domain performance of these MAPs with high domain specificity by design can be used to measure domain similarity. In this regard, we collected MAPs optimized on ImageNet $\rightarrow$ 10 datasets for 1-, 2-, 5-, and 10-shots. In total, we have 40 MAPs. We run these MAPs against 100-way $\{1, 2, 3, 5, 8, 10, 16, 20,32\}$-shot tasks on those 10 datasets. For the $i^{th}$ task with a specific combination of the number of shots and target domain, we compute the relative performance ranking of these 40 MAPs: $\vec{r}_i=\{r_{ij}\},j=1,\ldots,40$ . We visualize these $\vec{r}_i$ via t-SNE in Figure~\ref{fig:tsne}, using rank-correlation $\rho$ between $\vec{r}_i$ and $\vec{r}_j$ as the distance $d=\sqrt{1-\rho(\vec{r}_i,\vec{r}_j)}$. In so doing, domains that tend to favor the same set of adaptation methods would cluster in a closer neighborhood, as shown in Figure~\ref{fig:tsne}. We have the following insightful observations.  

%Figure 1 reveals several interesting points.
1) For each domain, varying the number of shots forms a continuous trajectory in the embedding space, suggesting that different adaptation methods are selected depending on the number of available labeled samples. 
%This means that increasing dataset size induces a smooth and predictable change in MAP configuration.

2) As the number of shots increases, trajectories from multiple domains converge to several attractors (highlighted by green circles in Figure~\ref{fig:tsne}). This is consistent with the observation that finetuning gradually emerges as the most effective adaptation method for high shots.

3) DomainNet-QDraw, FGVC-Aircraft and Traffic signs datasets emerge as a distinctive cluster. One signature that sets these datasets apart from others is that they all require recognition of strokes or silhouettes as opposed to textures. This also explains why it is difficult to generalize MAPs from other DomainNet datasets to DomainNet-QDraw (see cross-domain performance in Table~\ref{table:pipeline_generalization}). Towards further improving the effectiveness of hyperparameter transfer, having a set of diverse MAPs with sufficient coverage of the embedding space is desired.

%Similarly, we also created a TSNE embedding the dataset embedding space for finetuning in Figure 2 and it shows less detailed structure. This is because finetuning is more domain-agnostic. 

\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{fig/06-tsne.pdf}
    \label{fig:tsne}
    \caption{Domain similarity visualization using cross-domain performance of MAPs as the metric. Domains that favor similar MAPs form clusters.}
    \label{fig:tsne}
\end{figure}



%\begin{figure}[t]
%    \centering
%    \caption{\red{Placeholder for a from scratch vs transfer convergence rate plot}}
%    \includegraphics[width=1\textwidth]{fig/tsne.pdf}
%    \label{fig:hp_convergence}
%\end{figure}

==> Modular Adaptation ICCV2021 - Arxiv/ch/05-Conclusion.tex <==
%\vspace{-2mm}
\section{Conclusions}

We developed MAPs as an alternative to one-size-fits-all solutions for cross-domain FSL. Via MAP, We showed 1) that various adaptation methods can be unified under a common framework to achieve greater adaptation performance; and 2) that given a specific downstream task with limited training examples, which adaptation methods to apply can be configured and optimized dynamically and efficiently through hyperparameter transfer. Additionally, thanks to their domain specificity by design, the cross-domain performance of MAPs optimized for different domains revealed new perspectives to the similarity between domains. The effectiveness of MAPs was verified via an average $3.1\%$ improvement over finetuning on 5-shot ImageNet $\rightarrow$ 10 datasets benchmark and competitive performance against SOTA on LFT and VL3. Encouraged by these demonstrated advantages of MAP, promising directions for future research include speeding up online hyperparameter adaptation, improving hyperparameter generalization across datasets, and architectures and empirical rules for predicting hyperparameters.

==> Modular Adaptation ICCV2021 - Arxiv/fig/table01-main.tex <==
\begin{table*}[t]
\centering
\footnotesize
\tabcolsep=0.11cm
\noindent

\begin{tabular}{ c | l |c c c c c c | c c c c | c }
	\toprule
	 %\multicolumn{13}{c}{100-way K-shot ImageNet $\rightarrow$ 10 datasets }  \\
	& Approach & QDraw & Infgrph & Sketch & Clipart & Pnting & Real & CIFAR & Textures & Aircraft & Signs & Overall  \\
\midrule
\multirow{3}{*}{2-shot} &	PN   & 21.37 &  8.35 & 21.59 & 35.60 & 36.89 & 66.68 & 32.33 & 40.62 & 11.85 & 27.30 & 30.26  \\
	                    &   FT   & 31.88 &  8.61 & 22.68 & 35.54 & 34.22 & 57.02 & 28.87 & 30.40 & 16.61 & 58.37 & 32.42  \\
                   &\textbf{MAP} & 30.10 &  9.91 & 27.38 & 39.25 & 39.66 & 69.25 & 35.63 & 41.19 & 14.01 & 57.42 & \textbf{36.38}  \\
\midrule
\multirow{3}{*}{5-shot} &	PN    & 30.51 & 12.72 & 31.82 & 48.09 & 45.72 & 72.39 & 42.85 & 52.00 & 18.28 & 39.21  & 39.36  \\
	                    &   FT    & 47.29 & 14.26 & 39.02 & 54.05 & 50.42 & 71.26 & 47.25 & 46.47 & 35.94 & 87.56  & 49.35  \\
                   &\textbf{MAP}  & 45.73 & 16.49 & 43.23 & 59.21 & 55.21 & 74.94 & 55.97 & 52.15 & 36.13 & 85.74  & \textbf{52.48}  \\
		\midrule
\multirow{3}{*}{10-shot} &  PN    & 35.23 & 16.75 & 40.85 & 54.99 & 51.44 & 75.50 & 49.25 & 56.04 & 22.86 & 44.74 & 44.77  \\
	                    &   FT    & 58.14 & 20.00 & 48.88 & 65.98 & 58.22 & 77.05 & 59.54 & 56.22 & 51.51 & 92.79 & 58.83  \\
                   &\textbf{MAP}  & 55.33 & 23.64 & 49.74 & 68.45 & 59.70 & 77.66 & 61.50 & 54.36 & 53.34 & 94.06 & \textbf{59.78}  \\
		\midrule
\multirow{3}{*}{20-shot} &  PN   & 39.62 & 21.36 & 44.60 & 60.77 & 56.48 & 77.91 & 53.94 & 56.30 & 26.79 & 53.49 & 49.13  \\
	                    &   FT   & 66.04 & 26.89 & 56.58 & 72.96 & 64.97 & 80.61 & 68.14 & 62.77 & 72.25 & 96.44 & 66.77  \\
                   &\textbf{MAP} & 62.89 & 30.28 & 55.65 & 75.23 & 65.25 & 79.93 & 68.42 & 61.12 & 75.05 & 98.37 & \textbf{67.22}  \\
		\bottomrule
\end{tabular}

\caption{Comparing performance of MAP against PN and FT baselines on 100-way K-shot ImageNet $\rightarrow$ 10 datasets cross-domain few-shot learning benchmark. MAP outperforms PN/FT baselines by \{3.96, 3.13, 1.04, 0.44\}\% at \{2, 5, 10, 20\}-shots, respectively. }

%\vspace{-5pt}
\label{table:transfer}
\end{table*}


==> Modular Adaptation ICCV2021 - Arxiv/fig/table02-summary.tex <==
\begin{table*}[hbt!]
\centering
\footnotesize
\tabcolsep=0.11cm
\noindent

\begin{tabular}{ l |c c c c | c c c c | c c c c }
	\toprule
	%\multicolumn{13}{c}{DomainNet Overall accuracy using different hyperparameters} \\
	         & \multicolumn{4}{c}{From-scratch} & \multicolumn{4}{c}{Transfer} & \multicolumn{4}{c}{Oracle} \\
	Shots    &\bf{ MAP} & FT & PN & \bf{MAP vs FT/PN} & \bf{MAP} & FT & PN & \bf{MAP vs FT/PN} & \bf{MAP} & FT & PN & \bf{MAP vs FT/PN} \\
	\midrule
	2   & 36.15 & 31.36 & 31.81 & +4.34 &      35.93 & 31.66 & 31.75 & +4.18 &     36.34 & 30.74 & 32.30 & +4.04  \\
	5   & 47.70 & 44.14 & 40.77 & +3.56 &      49.14 & 46.05 & 40.21 & +3.09 &     49.00 & 46.28 & 41.06 & +2.72  \\
	10  & 55.84 & 54.14 & 46.61 & +1.70 &      55.75 & 54.71 & 45.79 & +1.04 &     55.92 & 55.07 & 46.61 & +0.85  \\
	20  & 61.30 & 61.22 & 50.34 & +0.08 &      61.54 & 61.34 & 50.12 & +0.20 &       -   &   -   &   -   &   -    \\
	\bottomrule
\end{tabular}

%\vspace{-5pt}

\caption{Comparing the performance of \emph{from-scratch} and \emph{transfer} hyperparameter selection strategies against the \emph{oracle} of 500 rounds of Bayesian hyperparameter optimization on 100-way K-shot ImageNet $\rightarrow$ DomainNet datasets. Both \emph{from-scratch} and \emph{transfer} can match the performance of \emph{oracle}. \emph{transfer} is more than 10x faster to run than \emph{from-scratch}.}

\label{table:summary}
\end{table*}


==> Modular Adaptation ICCV2021 - Arxiv/fig/table03-generalization.tex <==
\begin{table}[t]
\centering
\footnotesize
\tabcolsep=0.11cm
\begin{tabular}{ l |c c c c c c }
	\toprule
	      %\multicolumn{7}{c}{MAP generalization on DomainNet 5-shot tasks} \\
	MAP  & QDraw & Infgrph & Sketch & Clipart &  Pnting & Real \\
	\midrule
	DN-QDraw-5       & \bf{47.75} &      9.05  &     26.55  &     39.00  &     25.95  &     25.95      \\
	DN-Infgrph-5     &     38.15  &     14.80  &     38.15  &     48.80  &     46.40  &     70.45      \\
	DN-Sketch-5      &     42.65  &     17.20  & \bf{41.75} &     54.65  &     50.55  &     71.95      \\
	DN-Clipart-5     &     38.65  & \bf{17.50} &     41.45  &     56.75  & \bf{53.45} &     73.65      \\
	DN-Pnting-5      &     37.75  &     14.45  &     38.40  & \bf{56.80} &     52.40  & \bf{75.20}      \\
	DN-Real-5        &     33.95  &     16.05  &     39.05  &     54.10  &     49.70  &     73.15      \\
	\bottomrule
\end{tabular}
\caption{Cross-domain performance of six MAPs for 100-way 5-shot ImageNet $\rightarrow$ DomainNet tasks. %DN-Clipart-5 performs well on most datasets but underperforms on the QuickDraw domain. DN-QDraw-5 is particularly effective on QuickDraw but does not perform well in other domains, suggesting that different datasets favor different MAPs.
}

%Performance of 4 MAPs searched for 5-shot tasks in DomainNet Real, Clipart, Sketch and QuickDraw domains respectively, on unseen 5-shot tasks in other DomainNet domains. DomainNet-Clipart MAP has near-top performance across all domains except for QuickDraw, where as the DomainNet-QuickDraw MAP performs well on QuickDraw specifically but could not generalize to other DomainNet domains.

\label{table:pipeline_generalization}

\end{table}


==> Modular Adaptation ICCV2021 - Arxiv/fig/table04-vl3-lft.tex <==
\begin{table*}
\centering
\scriptsize
\tabcolsep=0.11cm
\noindent

%\begin{minipage}{1\textwidth}
\centering
	\begin{tabular}{ l | c c | c c c c }
		\toprule
%		 \multicolumn{7}{c}{5-way 5-shot LFT benchmark }  \\
		Approach & Arch. & Trans. & CUB & Cars & Places & Plantae   \\
		\midrule
		RelationNet                    & ResNet-10 &             & 57.77 $\pm$ 0.69      & 37.33 $\pm$ 0.68      & 63.32 $\pm$ 0.76      & 44.00 $\pm$ 0.60 \\
RelationNet+LFT~\cite{tseng2020cross}  & ResNet-10 &             & 59.46 $\pm$ 0.71      & 39.91 $\pm$ 0.69      & 66.28 $\pm$ 0.72      & 45.08 $\pm$ 0.59 \\
		GNN                            & GNN       & \Checkmark  & 62.25 $\pm$ 0.65      & 44.28 $\pm$ 0.63      & 70.84 $\pm$ 0.65      & 52.53 $\pm$ 0.59 \\
		GNN+LFT~\cite{tseng2020cross}  & GNN       & \Checkmark  & 66.98 $\pm$ 0.68      & 44.90 $\pm$ 0.64      & 73.94 $\pm$ 0.67      & 53.85 $\pm$ 0.62 \\
		\midrule
		PN                             & ResNet-10 & \Checkmark  & 66.48 $\pm$ 1.08      & 51.68 $\pm$ 1.16      & 73.66 $\pm$ 1.04      & 58.98 $\pm$ 1.12 \\
		FT                             & ResNet-10 & \Checkmark  & 67.31 $\pm$ 1.03      & \bf{51.89 $\pm$ 1.14} & 71.68 $\pm$ 1.02      & \bf{60.26 $\pm$ 1.09} \\
		\textbf{MAP}                   & ResNet-10 & \Checkmark  & \bf{67.92 $\pm$ 1.10} & 51.64 $\pm$ 1.16      & \bf{75.94 $\pm$ 0.97} & 58.45 $\pm$ 1.15 \\
		\bottomrule
	\end{tabular}
%\end{minipage}
%
%
%\vspace{-5pt}
\caption{Performance on 5-way 5-shot LFT benchmark.}


\label{table:LFT}
\end{table*}

\begin{table*}
\centering
\scriptsize
\tabcolsep=0.11cm
\noindent

%\begin{minipage}{1\textwidth}
\centering
	\begin{tabular}{ l |c c c c c c c c }
		\toprule
		  %\multicolumn{9}{c}{5-way 5/20-shot VL3 with pretrained ResNet-10 }  \\
		Approach & \multicolumn{2}{c}{CropDisease} & \multicolumn{2}{c}{EuroSAT} & \multicolumn{2}{c}{ISIC} & \multicolumn{2}{c}{ChestX}  \\
		         & 5-shot & 20-shot & 5-shot & 20-shot & 5-shot & 20-shot & 5-shot & 20-shot   \\
		\midrule
		Transductive FT~\cite{guo2020broader}& 90.64 $\pm$ 0.54      & 95.91 $\pm$ 0.72      & 81.76 $\pm$ 0.48      & 87.97 $\pm$ 0.42      & 49.68 $\pm$ 0.36      & 61.09 $\pm$ 0.44      & 26.09 $\pm$ 0.96      & 31.01 $\pm$ 0.59      \\
		FT + Data aug.~\cite{cai2020cross}   & \bf{92.23 $\pm$ 0.46} & 95.95 $\pm$ 0.30      & 82.67 $\pm$ 0.50      & 87.84 $\pm$ 0.46      & \bf{51.76 $\pm$ 0.50} & 60.32 $\pm$ 0.59      & \bf{31.60 $\pm$ 0.41} & \bf{35.91 $\pm$ 0.42} \\
		\midrule
		PN                                   & 90.10 $\pm$ 1.11      & 93.95 $\pm$ 0.84      & 80.49 $\pm$ 1.27      & 86.08 $\pm$ 1.00      & 44.73 $\pm$ 1.31      & 56.86 $\pm$ 1.18      & 24.31 $\pm$ 0.83      & 29.48 $\pm$ 0.83      \\
		FT                                   & 85.52 $\pm$ 1.37      & \bf{96.07 $\pm$ 0.75} & 79.93 $\pm$ 1.31      & \bf{89.93 $\pm$ 1.29} & 46.86 $\pm$ 1.29      & \bf{62.86 $\pm$ 1.62} & 24.29 $\pm$ 0.85      & 30.60 $\pm$ 1.09      \\
        \bf{MAP}                             & 90.29 $\pm$ 1.56      & 95.22 $\pm$ 1.13      & \bf{82.76 $\pm$ 2.00} & 88.11 $\pm$ 1.78      & 47.85 $\pm$ 1.95      & 60.16 $\pm$ 2.70      & 24.79 $\pm$ 1.22      & 30.21 $\pm$ 1.78      \\
		\bottomrule
	\end{tabular}
%\end{minipage}

%\vspace{-5pt}
\caption{Performance on 5-way 5- and 20-shot VL3 benchmark with ``single model finetuning''}


\label{table:VL3}
\end{table*}


==> Modular Adaptation ICCV2021 - Arxiv/fig/tableA1-full-results.tex <==


\begin{table*}[htbp!]
\centering
\footnotesize
\tabcolsep=0.11cm
\noindent

\begin{tabular}{ c " l " c c c c c c | c " c c c c " c }
	\toprule
	 \multicolumn{14}{c}{100-way K-shot ImageNet $\rightarrow$ 10 datasets under \emph{from-scratch} hyperparameters }  \\
	 \midrule
	& & \multicolumn{7}{c}{DomainNet} & CIFAR & Textures & Aircraft & Signs & Overall  \\
	& Approach & QDraw & Infgrph & Sketch & Clipart & Pnting & Real & Average &   &   &   &   &    \\
\midrule
\multirow{3}{*}{2-shot} &	PN   & 22.29 &  9.24 & 24.09 & 34.99 & 33.78 & 66.48 & 31.81 & 34.66 & 41.21 & 15.48 & 30.37 & 31.26  \\
	                    &   FT   & 31.42 &  8.85 & 23.10 & 32.40 & 32.38 & 59.98 & 31.36 & 33.31 & 34.68 & 19.79 & 61.28 & 33.72  \\
                   &\textbf{MAP} & 33.90 & 11.07 & 29.19 & 41.27 & 35.32 & 66.14 & 36.15 & 35.35 & 42.36 & 14.96 & 59.30 & \textbf{36.89}  \\
\midrule
\multirow{3}{*}{5-shot} &	PN   & 31.06 & 14.27 & 33.62 & 44.82 & 47.25 & 73.57 & 40.77 & 43.27 & 51.15 & 19.11 & 40.74  & 39.89  \\
	                    &   FT   & 47.29 & 15.23 & 26.84 & 54.38 & 48.68 & 72.42 & 44.14 & 50.46 & 47.47 & 36.68 & 83.65  & 48.31  \\
                   &\textbf{MAP} & 47.33 & 17.18 & 43.03 & 57.15 & 46.72 & 74.79 & 47.70 & 43.99 & 52.04 & 40.00 & 84.19  & \textbf{50.64}  \\
		\midrule
\multirow{3}{*}{10-shot} &  PN   & 37.08 & 17.53 & 41.02 & 55.71 & 52.68 & 75.64 & 46.61 & 51.40 & 55.38 & 24.31 & 47.12 & 45.79  \\
	                    &   FT   & 57.51 & 20.45 & 47.79 & 64.47 & 58.25 & 76.35 & 54.14 & 61.11 & 52.94 & 56.85 & 97.26 & 59.30  \\
                   &\textbf{MAP} & 58.05 & 22.06 & 51.26 & 66.69 & 59.86 & 77.14 & 55.84 & 59.77 & 54.23 & 54.71 & 96.63 & \textbf{60.04}  \\
		\midrule
\multirow{3}{*}{20-shot} &  PN   & 40.50 & 21.07 & 45.65 & 60.54 & 56.63 & 77.65 & 50.34 & 54.72 & 60.15 & 28.62 & 54.28 & 49.98  \\
	           &   \textbf{FT}   & 64.54 & 26.95 & 56.54 & 73.27 & 65.04 & 80.98 & 61.22 & 67.98 & 61.96 & 73.37 & 98.84 & \textbf{66.95}  \\
                   &         MAP & 64.13 & 28.62 & 58.03 & 72.33 & 64.58 & 80.08 & 61.30 & 67.05 & 63.15 & 71.15 & 98.65 & 66.81  \\
		\bottomrule
\end{tabular}

\begin{tabular}{ c " l " c c c c c c | c " c c c c " c }
	\toprule
	 \multicolumn{14}{c}{100-way K-shot ImageNet $\rightarrow$ 10 datasets under \emph{oracle} hyperparameters }  \\
	 \midrule
	& & \multicolumn{7}{c}{DomainNet} & CIFAR & Textures & Aircraft & Signs & Overall  \\
	& Approach & QDraw & Infgrph & Sketch & Clipart & Pnting & Real & Average &   &   &   &   &    \\
\midrule
\multirow{3}{*}{2-shot} &	PN    & 22.33 &  9.70 & 26.18 & 34.06 & 35.46 & 66.05 & 32.30 & 34.86 & 44.00 & 15.50 & 30.70  & 31.88  \\
	                    &   FT    & 30.62 &  7.98 & 21.42 & 31.43 & 33.54 & 59.43 & 30.74 & 31.46 & 35.43 & 19.79 & 58.67  & 32.98  \\
                   &\textbf{MAP}  & 31.52 & 11.52 & 31.39 & 39.76 & 36.57 & 67.27 & 36.34 & 33.74 & 44.19 & 22.80 & 53.84  & \textbf{37.26}  \\
		\midrule
\multirow{3}{*}{5-shot} &  PN     & 32.30 & 14.71 & 40.85 & 33.71 & 44.87 & 73.08 & 41.06 & 44.00 & 50.85 & 20.26 & 41.35 & 40.28  \\
	                    &   FT    & 48.12 & 15.32 & 48.88 & 37.94 & 49.23 & 72.43 & 46.28 & 45.74 & 46.38 & 38.93 & 92.12 & 50.08  \\
                   &\textbf{MAP}  & 48.99 & 15.42 & 49.74 & 41.82 & 54.70 & 74.88 & 49.00 & 50.89 & 52.43 & 39.36 & 93.03 & \textbf{52.97}  \\
		\midrule
\multirow{3}{*}{10-shot} &  PN    & 37.62 & 17.71 & 44.60 & 41.22 & 52.37 & 75.16 & 46.61 & 51.21 & 55.60 & 24.04 & 47.56 & 45.81  \\
	                    &   FT    & 57.57 & 21.38 & 56.58 & 48.71 & 59.12 & 76.99 & 55.07 & 60.84 & 55.55 & 55.18 & 97.12 & 59.91  \\
                   &\textbf{MAP}  & 58.49 & 22.26 & 55.65 & 52.30 & 58.27 & 76.84 & 55.92 & 61.83 & 54.72 & 58.81 & 97.23 & \textbf{60.81}  \\
		\bottomrule
\end{tabular}

\caption{Performance of PN/FT/MAP under \emph{from-scratch} and \emph{oracle setups}. Results on DomainNet datasets are averaged to create Table 4 in the main paper. }

%\vspace{-5pt}
\label{table:full_result}
\end{table*}


==> Modular Adaptation ICCV2021 - Arxiv/macros.tex <==

\newcommand{\paracompact}{\noindent\textbf}
\newcommand{\tb}{\textbf}
\newcommand{\red}{\textcolor{red}}

